Neural Variational Inference and Learning in Undirected Graphical Models

Many problems in machine learning are naturally expressed in the language of undirected graphical models. Here, we propose black-box learning and inference algorithms for undirected models that optimize a variational approximation to the log-likelihood of the model. Central to our approach is an upper bound on the log-partition function parametrized by a function q that we express as a flexible neural network. Our bound makes it possible to track the partition function during learning, to speed-up sampling, and to train a broad class of hybrid directed/undirected models via a unified variational inference framework. We empirically demonstrate the effectiveness of our method on several popular generative modeling datasets.

==> figures/Makefile <==
all:
	make figure.pdf

figure.pdf: out5b.txt
	python ./figure.py \
	  -d $< \
	  -f $@

figure-d7.pdf: ./out7b.txt
	python ./figure.py \
	  -d $< \
	  -f $@


==> framework.tex.bak.tex <==
\section{ONLINE RECALIBRATION}\label{sec:recalibration}

Notice that the above algorithm has two important shortcomings that make it inapplicable to the kind of calibrated prediction problems that we discussed earlier (e.g. medical diagnosis). First, this method is not applicable to the standard machine learning setting where we wish to predict $y_t$ from covariates $x_t$. Secondly, it only guarantees calibration, which by itself may not be enough: for example, predicting the average $\frac{1}{T}\sum_{t=1}^T y_t$ (assuming its limit exists) will result in a calibrated but useless algorithm. In order to be useful, our predictions must also effectively predict $y_t$.

Here, we define a new problem called {\em online recalibration} that addresses these shortcomings. We propose transforming a sequence of {\em uncalibrated} forecasts $\palg_t$ into predictions $p_t$ that are calibrated and as accurate as the original $\palg_t$. The forecasts $\palg_t$ may come from any existing machine learning system $F$; our methods will not alter this system, and if it possesses favorable convergence properties (e.g. the ability to exploit sparsity or seed up its convergence via adaptive learning rates like Adagrad), our calibrated $p_t$ will inherit all of these properties.

We now formalize the online recalibration problem. At every step $t=1,...,T$:
\begin{enumerate}
\item Nature chooses $(x_t, y_t) \in \Xc \times \{0, 1\}$ and reveals $x_t \in \Xc \subseteq \Rb^d$.
\item Forecaster $F$ predicts $\palg_t = \sigma (w_{t-1} \cdot x) \in [0,1]$.
\item A recalibration algorithm $A : [0,1] \to [0,1]$ produces a calibrated probability $p_t = A(\palg_t)$.
\item Nature reveals $y_t$; $F$ incurs loss of $\ell(p_t , y_t)$, where $\ell : \Pc \times \Yc \to \Rb^+$ is a convex loss function.
\item $F$ updates $w_t$; $A$ updates itself based on $y_t$.
\end{enumerate}

\begin{defn}
We say that $A$ is an $\e$-accurate online recalibration algorithm if
\begin{itemize}
\item The forecasts $p_t = A(\palg_t)$ are $\e$-calibrated.
\item The regret of $p_t$ with respect to $\palg_t$ is small:  $\lim_{T \to \infty} \frac{1}{T} \sum_{t=1}^T \left( \ell(p_t , y_t) - \ell(\palg_t , y_t)\right) \leq \epsilon.$
\end{itemize}
\end{defn}

\section{RECALIBRATION FRAMEWORK}\label{sec:framework}

Now that we have defined the online recalibration problem, we turn our attention to constructing an $\e$-accurate algorithm. In \algorithmref{recal}, we introduce a general framework that accepts an online calibration algorithm $\Fcal$ such as \algorithmref{online_cal} and uses it as a black box within a simple procedure that yields an $\e$-accurate online recalibration algorithm.

\begin{algorithm}[t]
  \caption{Recalibration framework}
  \label{algo:recal}
  \begin{algorithmic}[1]
    \REQUIRE Number of buckets $M$, online calibration algorithm $\Fcal$, uncalibrated forecasts $(\palg_t)_{t=1}^T$.
    \STATE Let $\Ic = \{[0,\frac{1}{M}), [\frac{1}{M}, \frac{2}{M}), ..., [\frac{M-1}{M},1]\}$ be a set of intervals that partition $[0,1]$.
    \STATE Let $\Fc = \{ \Fcal_j \mid i = 0,...,M-1 \}$ be a set of $M$ independent instances of $\Fcal.$
    \FOR {$t=1,...,T$:}
    \STATE Let $[\frac{j}{M}, \frac{j+1}{M})$ be the interval containing $\palg_t$.
    \STATE Let $p_t$ be the forecast of $\Fcal_j \in \Fc$. Output $p_t$.
    \STATE Observe $y_t$ and pass it to $\Fcal_j \in \Fc$.
    \ENDFOR
  \end{algorithmic}
\end{algorithm}

\algorithmref{recal} partitions the sequence $(y_t)_{t=1}^T$ into $M$ disjoint sets $S_j = \{ y_t \mid \palg_t \in [\frac{j}{M}, \frac{j+1}{M}) \}$ for $j=0,1,...,M-1$ and trains a separate $\Fcal_j$ on each set $S_j$. After observing $\palg_t$, \algorithmref{recal}  outputs the prediction of the $\Fcal_i$ associated with the interval $[\frac{j}{M}, \frac{j+1}{M}) \ni \palg_t$. One can show that with sufficiently high resolution, $\Fcal_j$ is guaranteed to do as well as constantly predicting $\frac{j}{M}$ (it turns out that $\Fcal_j$ also minimizes external regret). By construction, whenever $\Fcal_j$ is called, $\palg_t \approx \frac{j}{M}$ and so we are guaranteed to do about as well as $\palg_t$; since this is true for any $j$, we will do at least as well as $\palg_t$ on the entire input sequence.

Note that the above construction is directly inspired by the histogram method for recalibrating probabilities in the batch setting. The histogram method splits the $(y_t, \palg_t)$ into $M$ disjoint bins $B_i = \{ (y_t, \palg_t) \mid \palg_t \in [\frac{j}{M}, \frac{j+1}{M}) \}$ for $j=0,1,...,M-1$ and predicts the average $y_t$ in each bin. If the $(y_t, \palg_t)$ are sampled i.i.d. from some $\Pb$, then the bin averages are guaranteed to converge to $ \Pb(y=1 \mid \palg_t \in [\frac{j}{M}, \frac{j+1}{M})). $ 
%This construction assumes that  $\Pb(y=1 \mid \palg_t)$ is lower for smaller $\palg_t$ and also gives us the freedom to predict $i/M$ on each interval, which corresponds to predicting the original $\palg_t$.
In the online setting, the $y_t$ may be adversarial and hence we cannot simply output the average of each interval. However, we can achieve the same effect by instead using an online calibrated predictor.

\subsection{Algorithm correctness}

Having defined and motivated our method, we now proceed to show that it is indeed $\e$-accurate.
Suppose that each subroutine $\Fcal_j$ has resolution $1/N$ and let $w^A_1, w^A_2,...$ be the random distributions over $\{\frac{i}{N} \mid i =0,...,N\}$ generated by \algorithmref{recal}.

Let also
$ \tilde \rho_T(i/N) = \frac{\sum_{t=1}^T y_t w^A_{t,i}}{\sum_{t=1}^T w^A_{t,i}} $
and
$$ \tilde C_T = \sum_{i=0}^N \left( \tilde \rho_n(i/N) - \frac{i}{N} \right)^2 \left( \frac{1}{T} \sum_{t=1}^T w^A_{t,i} \right) $$
be the corresponding values of $\rho_T$ and $C_T$ ``in expectation".
Note that by standard convergence results, one can show that
$ \lim_{T \to \infty} \left | \frac{1}{T}\sum_{t=1}^T \Ind_{I_t = i} - \sum_{t=1}^T p^A_{t,i} \right| \to 0, $
based on which, we can establish the following lemma
\begin{lemma}
We have $\lim_{T \to \infty} C_T = \tilde C_T$.\qed
\end{lemma}
We state the full proof of the lemma in the appendix. Note however that to analyze \algorithmref{recal}, it now sufficient to work with $\tilde \rho_T(i/N)$ and $\tilde C_T$.

Next, let
$$
\wsupi_{t,j} = \begin{cases}
\textrm{prediction of $\Fcal_i$} & \textrm{if $\palg \in [\frac{i}{N}, \frac{i+1}{N})$} \\
0 & \textrm{otherwise}.
\end{cases}
$$
Note that $p^A_t = \sum_{i=1}^N \wsupi_t \Ind_{\palg \in I_i}$. 
Furthermore, let
\begin{align*}
& \rit(j/M) = \frac{\sum_{t=1}^T \wsupi_{t,j} y_t}{\sum_{t=1}^T \wsupi_{t,j}}
& \tilde \rho_T(j/M) = \frac{\sum_{t=1}^T p^A_{t,j} y_t}{\sum_{t=1}^T p^A_{t,j}} 
%= \frac{\sum_{i=1}^N \sum_{t=1}^T \wsupi_{t,j} y_t}{\sum_{i=1}^N \sum_{t=1}^T \wsupi_{t,j}} 
\end{align*}
be (respectively) the empirical observation frequencies of $y_t$ for $\Fcal_i$ and for $A$. 
%Let also
%\begin{align*}
%& \wi_j = \sum_{t=1}^T \wsupi_{t,j}
%& w_j = \sum_{t=1}^T p^A_{t,j} =  \sum_{i=1}^N \sum_{t=1}^T \wsupi_{t,j} = \sum_{i=1}^N \wi_j.
%\end{align*}
Finally, let $\tilde C^{(i)}_{T} \sum_{j=1}^T C^{(i)}_{T,j}$ and $\tilde C_{T} = \sum_{j=1}^T C_{T,j}$ denote respectively the calibration values of $\Fcal_i$ and of the main algorithm, where
\begin{align*}
\tilde C^{(i)}_{T,j} & = \left( \rit(j/M) - \frac{j}{M} \right)^2 \left( \frac{1}{T} \sum_{t=1}^T \wsupi_{t,j} \right) \\
\tilde C_{T,j} & = \left( \tilde \rho_T(j/M) - \frac{j}{M} \right)^2 \left( \frac{1}{T} \sum_{t=1}^T p^A_{t,j} \right).
\end{align*}

\begin{lemma}
Choose $N$ such that $1/N < \e$. If each $\Fcal$ is $\e$-calibrated then \algorithmref{recal} with $N$ and $\Fcal$ is and $\e$-accurate recalibration algorithm.
\end{lemma}

\begin{proof}
Notice that we can write
\begin{align*}
& \tilde C_{T,j} 
 = \frac{\sum_{t=1}^T p^A_{t,j}}{T} \left( \tilde \rho_T(j/M) - \frac{j}{M} \right)^2 \\
& \;\;\;\; = \frac{\sum_{i=1}^N \sum_{t=1}^T \wsupi_{t,j}}{T} \left( \frac{\sum_{i=1}^N \sum_{t=1}^T \wsupi_{t,j} y_t}{\sum_{i=1}^N \sum_{t=1}^T \wsupi_{t,j}}  - \frac{j}{M} \right)^2 \\
%& = \left( \sum_{i=1}^N \frac{\wi_j}{T} \right) \left( \frac{\sum_{i=1}^N \wi_j \rit(j/M) }{\sum_{i=1}^N \wi_j }  - \frac{j}{M} \right)^2 \\
& \;\;\;\; \leq \sum_{i=1}^N \frac{\sum_{t=1}^T \wsupi_{t,j}}{T} \left( \rit(j/M) - \frac{j}{M} \right)^2 = \sum_{i=1}^N  \frac{T_i}{T}\tilde C^{(i)}_{T_i,j},
\end{align*}
where the last inequality follows by Jensen's and where $T_i$ is the number of plays of $\Fcal_i$. 
By our results for the previous algorithm, we find that
\begin{align*}
\tilde C_T 
& = \sum_{j=1}^M \tilde C_{T,j}
\leq \sum_{i=1}^N \sum_{j=1}^M \frac{T_i}{T} C^{(i)}_{T,j} \\
& \leq \sum_{i=1}^N \frac{T_i}{T} R_{T_i} + \e.
\end{align*}
Since $R_{T_i} \to 0$, the claim follows.
\end{proof}

\begin{lemma}
The recalibrated forecasts $p_t$ are not worse than the $\palg_t$ in the sense that
$$ \lim_{T\to\infty} \left( \frac{1}{T} \sum_{t=1}^T (y_t - p_t)^2 - \frac{1}{T} \sum_{t=1}^T (y_t - \palg_t)^2 \right) < 1/N. $$
\end{lemma}

\begin{proof}
Observe that we can write
\begin{align*}
\frac{1}{T}  &\sum_{t=1}^T  (y_t - p_t)^2 - \frac{1}{T} \sum_{t=1}^T (y_t - \palg_t)^2 \\
& = \frac{1}{T} \sum_{t=1}^T \left( \sum_{i=1}^N \left( (y_t - p_t)^2 - (y_t - \palg_t)^2 \right) \Ind_{\palg_t \in I_i} \right) \\
& < \frac{1}{T} \sum_{t=1}^T \left( \sum_{i=1}^N \left( (y_t - p_t)^2 - (y_t - \frac{i}{N})^2 \right) \Ind_{\palg_t \in I_i} + \frac{1}{N^2}\right) \\
& \leq \frac{1}{T} \sum_{t=1}^T \sum_{i=1}^N \frac{T_i}{T} R^{(i)}_{i,T_i} + \frac{1}{N^2},
\end{align*}
where $R^{(i)}_{i,T_i}$ is the external regret of algorithm $i$ with respect to action $i/N$ after $T_i$ plays.
The first inequality follows from the fact that each time $\palg_i \in I_i$, we can replace $(y_t - \palg_t)^2$ by $(y_t - i/N)^2$ resulting in a loss of precision of at most $1/N^2$ (because we choose all the intervals in $\Ic$ to be of size $1/N$). For the second inequality, we simply use the definition of regret (since $N=M$, $i/N$ is a valid constant action within algorithm $i$).
\end{proof}

\vk{TODO: Work our the case of different losses (not just $\ell_2$) and how it affects the rate. Currently, we actually just need to use $\sqrt{N}$ bins with the $\ell_2$ loss. Need to work this out.}

\subsection{Convergence rates}

For all calibration algorithms $\Fcal$ that we know of, we can write,
$R^{(i)}_{T_i} \leq f(\e)/\sqrt{T_i}$ for some $f(\e)$.
Therefore,
$$ \sum_{i=1}^N \frac{T_i}{T} R_{T_i} \leq \sum_{i=1}^N \frac{\sqrt{T_i}f(\e)}{T} \leq \frac{f(\e)}{\sqrt{ \e T}}, $$
where we used the fact that  $1 / N < \e.$
Thus, the recalibration procedure adds an extra
$ \frac{1}{\sqrt{\e}} $
term to the convergence rate as well as an extra $ \frac{1}{{\e}} $ term to the memory requirements. However, the per-iteration running time of the recalibraiton algorithm remains the same, because at each time step, we only activate a single $\Fcal_i$.
Note also that by the same argument, an extra $1/\sqrt{\e}$ is added to the convergence rate of the regret $ \frac{1}{T} \sum_{t=1}^T (y_t - p_t)^2 - \frac{1}{T} \sum_{t=1}^T (y_t - \palg_t)^2 $ w.r.t. $\palg$.

The most efficient calibration algorithm for the binary case is currently the one Abernethy, et al.~(2011). It has $O(\log(\frac{1}{\e}))$ running time per iteration, uses $O(1/{\e})$ memory, and converges at a rate of $O(\frac{1}{\sqrt{\e T}})$. Instantiated within our framework, this leads to a recalibration algorithm with $O(\log(\frac{1}{\e}))$ running time per iteration, $O(1/\e)$ memory usage, $O(1/(\e \sqrt{T}))$ convergence rate.

However, we believe that in practice practitioners will most likely use \algorithmref{online_cal}, as it is considerably simpler than that of Abernethy, et al. Instantiated within our framework, that method leads to a recalibration algorithm with $O(\log(1/\e))$ running time per iteration, $O(1/\e\sqrt{\e})$ memory usage, $O(1/(\e \sqrt{\e T}))$ convergence rate.

%In the $K$-label setting, all existing algorithms run in $O(1/\e^K)$ time/space and converges at a rate of $O(1/(\e^K \sqrt{T}))$. Instantiated with our method, this leads to:
%\begin{itemize}
%\item $O(1/\e^K)$ running time per iteration
%\item $O(1/\e^{K+1})$ memory usage
%\item $O(1/(\e^{K+1} T))$ convergence rate
%\end{itemize}

\subsection{Calibration with advice from multiple experts}

Next, consider the question of producing calibrated predictions with $K$ side experts each making their predictions $\pk$. A naive approach would be to discretize the space $[0,1]^K$ of their predictions.

Instead, given the predictions $\pk$, we first run an external regret minimization algorithm to produce a forecast $\palg$ that has a regret of $R_{\textrm{ext}, T}$ satisfying
$$ R_{\textrm{ext}, T} \geq \frac{1}{T} \sum_{t=1}^T (y_t - \palg_t)^2 - \frac{1}{T} \sum_{t=1}^T (y_t - \pk_t)^2 $$ 
with respect to each $\pk$. Then for each $k \in [K]$ the regret of our calibrated algorithm can be expressed as:
\begin{align*}
\frac{1}{T} & \sum_{t=1}^T (y_t - p_t)^2 
\leq \frac{1}{T} \sum_{t=1}^T (y_t - \palg_t)^2 + \frac{1}{T} \sum_{t=1}^T \sum_{i=1}^N R^{(i)}_{i,T_i} + \frac{1}{N} \\
& \leq \frac{1}{T} \sum_{t=1}^T (y_t - \pk_t)^2 + \frac{R_{\textrm{ext}, T}}{T} + \frac{1}{T} \sum_{t=1}^T \sum_{i=1}^N R^{(i)}_{i,T_i} + \frac{1}{N}.
\end{align*}

Typically, $R_{\textrm{ext}, T} = O(1/\sqrt{T})$, and we therefore get the same $O(1/\sqrt{T})$ regret for each $\pk$ as we did when $K=1$.

The dependence on $K$ depends on the external regret minimization algorithm that we use; it can be made as low as $O(\sqrt{(\log K) / T})$. Note that we factored out the dependence on $K$ from our framework, and so our dependence on $K$ can be made equal to that of the current best algorithm.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{ONLINE RECALIBRATION}\label{sec:recalibration}

Notice that the above algorithm has two important shortcomings that make it inapplicable to the kind of calibrated prediction problems that we discussed earlier (e.g. medical diagnosis). First, this method is not applicable to the standard machine learning setting where we wish to predict $y_t$ from covariates $x_t$. Secondly, it only guarantees calibration, which by itself may not be enough: for example, predicting the average $\frac{1}{T}\sum_{t=1}^T y_t$ (assuming its limit exists) will result in a calibrated but useless algorithm. In order to be useful, our predictions must also effectively predict $y_t$.

Here, we define a new problem called {\em online recalibration} that addresses these shortcomings. We propose transforming a sequence of {\em uncalibrated} forecasts $\palg_t$ into predictions $p_t$ that are calibrated and as accurate as the original $\palg_t$. The forecasts $\palg_t$ may come from any existing machine learning system $F$; our methods will not alter this system, and if it possesses favorable convergence properties (e.g. the ability to exploit sparsity or seed up its convergence via adaptive learning rates like Adagrad), our calibrated $p_t$ will inherit all of these properties.

We now formalize the online recalibration problem. At every step $t=1,...,T$:
\begin{enumerate}
\item Nature chooses $(x_t, y_t) \in \Xc \times \{0, 1\}$ and reveals $x_t \in \Xc \subseteq \Rb^d$.
\item Forecaster $F$ predicts $\palg_t = \sigma (w_{t-1} \cdot x) \in [0,1]$.
\item A recalibration algorithm $A : [0,1] \to [0,1]$ produces a calibrated probability $p_t = A(\palg_t)$.
\item Nature reveals $y_t$; $F$ incurs loss of $\ell(p_t , y_t)$, where $\ell : \Pc \times \Yc \to \Rb^+$ is a convex loss function.
\item $F$ updates $w_t$; $A$ updates itself based on $y_t$.
\end{enumerate}

\begin{defn}
We say that $A$ is an $\e$-accurate online recalibration algorithm if
\begin{itemize}
\item The forecasts $p_t = A(\palg_t)$ are $\e$-calibrated.
\item The regret of $p_t$ with respect to $\palg_t$ is small:  $\lim_{T \to \infty} \frac{1}{T} \sum_{t=1}^T \left( \ell(p_t , y_t) - \ell(\palg_t , y_t)\right) \leq \epsilon.$
\end{itemize}
\end{defn}

\section{RECALIBRATION FRAMEWORK}\label{sec:framework}

Now that we have defined the online recalibration problem, we turn our attention to constructing an $\e$-accurate algorithm. In \algorithmref{recal}, we introduce a general framework that accepts an online calibration algorithm $\Fcal$ such as \algorithmref{online_cal} and uses it as a black box within a simple procedure that yields an $\e$-accurate online recalibration algorithm.

\begin{algorithm}[t]
  \caption{Recalibration framework}
  \label{algo:recal}
  \begin{algorithmic}[1]
    \REQUIRE Number of buckets $N$, online calibration algorithm $\Fcal$, uncalibrated forecasts $(\palg_t)_{t=1}^T$.
    \STATE Let $\Ic = \{[0,\frac{1}{N}), [\frac{1}{N}, \frac{2}{N}), ..., [\frac{N-1}{N},1]\}$ be a set of intervals that partition $[0,1]$.
    \STATE Let $\Fc = \{ \Fcal_i \mid i = 0,...,N-1 \}$ be a set of $N$ independent instances of $\Fcal.$
    \FOR {$t=1,...,T$:}
    \STATE Let $[\frac{i}{N}, \frac{i+1}{N})$ be the interval containing $\palg_t$.
    \STATE Let $p_t$ be the forecast of $\Fcal_i \in \Fc$. Output $p_t$.
    \STATE Observe $y_t$ and pass it to $\Fcal_i \in \Fc$.
    \ENDFOR
  \end{algorithmic}
\end{algorithm}

\algorithmref{recal} partitions the sequence $(y_t)_{t=1}^T$ into $N$ disjoint sets $S_i = \{ y_t \mid \palg_t \in [\frac{i}{N}, \frac{i+1}{N}) \}$ for $i=0,1,...,N-1$ and trains a separate $\Fcal_i$ on each set $S_i$. After observing $\palg_t$, \algorithmref{recal}  outputs the prediction of the $\Fcal_i$ associated with the interval $[\frac{i}{N}, \frac{i+1}{N}) \ni \palg_t$. One can show that $\Fcal_i$ is guaranteed to do as well as constantly predicting $\frac{i}{N}$ (it turns out that $\Fcal_i$ also minimizes external regret). By construction, whenever $\Fcal_i$ is called, $\palg_t \approx \frac{i}{N}$ and so we are guaranteed to do about as well as $\palg_t$; since this is true for any $i$, we will do at least as well as $\palg_t$ on the entire input sequence.

Note that the above construction is directly inspired by the histogram method for recalibrating probabilities in the batch setting. The histogram method splits the $(y_t, \palg_t)$ into $N$ disjoint bins $B_i = \{ (y_t, \palg_t) \mid \palg_t \in [\frac{i}{N}, \frac{i+1}{N}) \}$ for $i=0,1,...,N-1$ and predicts the average $y_t$ in each bin. If the $(y_t, \palg_t)$ are sampled i.i.d. from some $\Pb$, then the bin averages are guaranteed to converge to $ \Pb(y=1 \mid \palg_t \in [\frac{i}{N}, \frac{i+1}{N})). $ 
%This construction assumes that  $\Pb(y=1 \mid \palg_t)$ is lower for smaller $\palg_t$ and also gives us the freedom to predict $i/N$ on each interval, which corresponds to predicting the original $\palg_t$.
In the online setting, the $y_t$ may be adversarial and hence we cannot simply output the average of each interval. However, we can achieve the same effect by instead using an online calibrated predictor.

\subsection{Algorithm correctness}

Having defined and motivated our method, we now proceed to show that it is indeed $\e$-accurate.
Suppose that each subroutine $\Fcal_j$ has resolution $1/N$ and let $w^A_1, w^A_2,...$ be the random distributions over $\{\frac{i}{N} \mid i =0,...,N\}$ generated by \algorithmref{recal}.

Let also
$ \tilde \rho_T(i/N) = \frac{\sum_{t=1}^T y_t w^A_{t,i}}{\sum_{t=1}^T w^A_{t,i}} $
and
$$ \tilde C_T = \sum_{i=0}^N \left( \tilde \rho_n(i/N) - \frac{i}{N} \right)^2 \left( \frac{1}{T} \sum_{t=1}^T w^A_{t,i} \right) $$
be the corresponding values of $\rho_T$ and $C_T$ ``in expectation".
Note that by standard convergence results, one can show that
$ \lim_{T \to \infty} \left | \frac{1}{T}\sum_{t=1}^T \Ind_{I_t = i} - \sum_{t=1}^T p^A_{t,i} \right| \to 0, $
based on which, we can establish the following lemma
\begin{lemma}
We have $\lim_{T \to \infty} C_T = \tilde C_T$.\qed
\end{lemma}
We state the full proof of the lemma in the appendix. Note however that to analyze \algorithmref{recal}, it now sufficient to work with $\tilde \rho_T(i/N)$ and $\tilde C_T$.

Next, let
$$
\wsupi_{t,j} = \begin{cases}
\textrm{prediction of $\Fcal_i$} & \textrm{if $\palg \in [\frac{i}{N}, \frac{i+1}{N})$} \\
0 & \textrm{otherwise}.
\end{cases}
$$
Note that $p^A_t = \sum_{i=1}^N \wsupi_t \Ind_{\palg \in I_i}$. 
Furthermore, let
\begin{align*}
& \rit(j/M) = \frac{\sum_{t=1}^T \wsupi_{t,j} y_t}{\sum_{t=1}^T \wsupi_{t,j}}
& \tilde \rho_T(j/M) = \frac{\sum_{t=1}^T p^A_{t,j} y_t}{\sum_{t=1}^T p^A_{t,j}} 
%= \frac{\sum_{i=1}^N \sum_{t=1}^T \wsupi_{t,j} y_t}{\sum_{i=1}^N \sum_{t=1}^T \wsupi_{t,j}} 
\end{align*}
be (respectively) the empirical observation frequencies of $y_t$ for $\Fcal_i$ and for $A$. 
%Let also
%\begin{align*}
%& \wi_j = \sum_{t=1}^T \wsupi_{t,j}
%& w_j = \sum_{t=1}^T p^A_{t,j} =  \sum_{i=1}^N \sum_{t=1}^T \wsupi_{t,j} = \sum_{i=1}^N \wi_j.
%\end{align*}
Finally, let $\tilde C^{(i)}_{T} \sum_{j=1}^T C^{(i)}_{T,j}$ and $\tilde C_{T} = \sum_{j=1}^T C_{T,j}$ denote respectively the calibration values of $\Fcal_i$ and of the main algorithm, where
\begin{align*}
\tilde C^{(i)}_{T,j} & = \left( \rit(j/M) - \frac{j}{M} \right)^2 \left( \frac{1}{T} \sum_{t=1}^T \wsupi_{t,j} \right) \\
\tilde C_{T,j} & = \left( \tilde \rho_T(j/M) - \frac{j}{M} \right)^2 \left( \frac{1}{T} \sum_{t=1}^T p^A_{t,j} \right).
\end{align*}

\begin{lemma}
Choose $N$ such that $1/N < \e$. If each $\Fcal$ is $\e$-calibrated then \algorithmref{recal} with $N$ and $\Fcal$ is and $\e$-accurate recalibration algorithm.
\end{lemma}

\begin{proof}
Notice that we can write
\begin{align*}
& \tilde C_{T,j} 
 = \frac{\sum_{t=1}^T p^A_{t,j}}{T} \left( \tilde \rho_T(j/M) - \frac{j}{M} \right)^2 \\
& \;\;\;\; = \frac{\sum_{i=1}^N \sum_{t=1}^T \wsupi_{t,j}}{T} \left( \frac{\sum_{i=1}^N \sum_{t=1}^T \wsupi_{t,j} y_t}{\sum_{i=1}^N \sum_{t=1}^T \wsupi_{t,j}}  - \frac{j}{M} \right)^2 \\
%& = \left( \sum_{i=1}^N \frac{\wi_j}{T} \right) \left( \frac{\sum_{i=1}^N \wi_j \rit(j/M) }{\sum_{i=1}^N \wi_j }  - \frac{j}{M} \right)^2 \\
& \;\;\;\; \leq \sum_{i=1}^N \frac{\sum_{t=1}^T \wsupi_{t,j}}{T} \left( \rit(j/M) - \frac{j}{M} \right)^2 = \sum_{i=1}^N  \frac{T_i}{T}\tilde C^{(i)}_{T_i,j},
\end{align*}
where the last inequality follows by Jensen's and where $T_i$ is the number of plays of $\Fcal_i$. 
By our results for the previous algorithm, we find that
\begin{align*}
\tilde C_T 
& = \sum_{j=1}^M \tilde C_{T,j}
\leq \sum_{i=1}^N \sum_{j=1}^M \frac{T_i}{T} C^{(i)}_{T,j} \\
& \leq \sum_{i=1}^N \frac{T_i}{T} R_{T_i} + \e.
\end{align*}
Since $R_{T_i} \to 0$, the claim follows.
\end{proof}

\begin{lemma}
The recalibrated forecasts $p_t$ are not worse than the $\palg_t$ in the sense that
$$ \lim_{T\to\infty} \left( \frac{1}{T} \sum_{t=1}^T (y_t - p_t)^2 - \frac{1}{T} \sum_{t=1}^T (y_t - \palg_t)^2 \right) < 1/N. $$
\end{lemma}

\begin{proof}
Observe that we can write
\begin{align*}
\frac{1}{T}  &\sum_{t=1}^T  (y_t - p_t)^2 - \frac{1}{T} \sum_{t=1}^T (y_t - \palg_t)^2 \\
& = \frac{1}{T} \sum_{t=1}^T \left( \sum_{i=1}^N \left( (y_t - p_t)^2 - (y_t - \palg_t)^2 \right) \Ind_{\palg_t \in I_i} \right) \\
& < \frac{1}{T} \sum_{t=1}^T \left( \sum_{i=1}^N \left( (y_t - p_t)^2 - (y_t - \frac{i}{N})^2 \right) \Ind_{\palg_t \in I_i} + \frac{1}{N^2}\right) \\
& \leq \frac{1}{T} \sum_{t=1}^T \sum_{i=1}^N \frac{T_i}{T} R^{(i)}_{i,T_i} + \frac{1}{N^2},
\end{align*}
where $R^{(i)}_{i,T_i}$ is the external regret of algorithm $i$ with respect to action $i/N$ after $T_i$ plays.
The first inequality follows from the fact that each time $\palg_i \in I_i$, we can replace $(y_t - \palg_t)^2$ by $(y_t - i/N)^2$ resulting in a loss of precision of at most $1/N^2$ (because we choose all the intervals in $\Ic$ to be of size $1/N$). For the second inequality, we simply use the definition of regret (since $N=M$, $i/N$ is a valid constant action within algorithm $i$).
\end{proof}

\vk{TODO: Work our the case of different losses (not just $\ell_2$) and how it affects the rate. Currently, we actually just need to use $\sqrt{N}$ bins with the $\ell_2$ loss. Need to work this out.}

\subsection{Convergence rates}

For all calibration algorithms $\Fcal$ that we know of, we can write,
$R^{(i)}_{T_i} \leq f(\e)/\sqrt{T_i}$ for some $f(\e)$.
Therefore,
$$ \sum_{i=1}^N \frac{T_i}{T} R_{T_i} \leq \sum_{i=1}^N \frac{\sqrt{T_i}f(\e)}{T} \leq \frac{f(\e)}{\sqrt{ \e T}}, $$
where we used the fact that  $1 / N < \e.$
Thus, the recalibration procedure adds an extra
$ \frac{1}{\sqrt{\e}} $
term to the convergence rate as well as an extra $ \frac{1}{{\e}} $ term to the memory requirements. However, the per-iteration running time of the recalibraiton algorithm remains the same, because at each time step, we only activate a single $\Fcal_i$.
Note also that by the same argument, an extra $1/\sqrt{\e}$ is added to the convergence rate of the regret $ \frac{1}{T} \sum_{t=1}^T (y_t - p_t)^2 - \frac{1}{T} \sum_{t=1}^T (y_t - \palg_t)^2 $ w.r.t. $\palg$.

The most efficient calibration algorithm for the binary case is currently the one Abernethy, et al.~(2011). It has $O(\log(\frac{1}{\e}))$ running time per iteration, uses $O(1/{\e})$ memory, and converges at a rate of $O(\frac{1}{\sqrt{\e T}})$. Instantiated within our framework, this leads to a recalibration algorithm with $O(\log(\frac{1}{\e}))$ running time per iteration, $O(1/\e)$ memory usage, $O(1/(\e \sqrt{T}))$ convergence rate.

However, we believe that in practice practitioners will most likely use \algorithmref{online_cal}, as it is considerably simpler than that of Abernethy, et al. Instantiated within our framework, that method leads to a recalibration algorithm with $O(\log(1/\e))$ running time per iteration, $O(1/\e\sqrt{\e})$ memory usage, $O(1/(\e \sqrt{\e T}))$ convergence rate.

%In the $K$-label setting, all existing algorithms run in $O(1/\e^K)$ time/space and converges at a rate of $O(1/(\e^K \sqrt{T}))$. Instantiated with our method, this leads to:
%\begin{itemize}
%\item $O(1/\e^K)$ running time per iteration
%\item $O(1/\e^{K+1})$ memory usage
%\item $O(1/(\e^{K+1} T))$ convergence rate
%\end{itemize}

\subsection{Calibration with advice from multiple experts}

Next, consider the question of producing calibrated predictions with $K$ side experts each making their predictions $\pk$. A naive approach would be to discretize the space $[0,1]^K$ of their predictions.

Instead, given the predictions $\pk$, we first run an external regret minimization algorithm to produce a forecast $\palg$ that has a regret of $R_{\textrm{ext}, T}$ satisfying
$$ R_{\textrm{ext}, T} \geq \frac{1}{T} \sum_{t=1}^T (y_t - \palg_t)^2 - \frac{1}{T} \sum_{t=1}^T (y_t - \pk_t)^2 $$ 
with respect to each $\pk$. Then for each $k \in [K]$ the regret of our calibrated algorithm can be expressed as:
\begin{align*}
\frac{1}{T} & \sum_{t=1}^T (y_t - p_t)^2 
\leq \frac{1}{T} \sum_{t=1}^T (y_t - \palg_t)^2 + \frac{1}{T} \sum_{t=1}^T \sum_{i=1}^N R^{(i)}_{i,T_i} + \frac{1}{N} \\
& \leq \frac{1}{T} \sum_{t=1}^T (y_t - \pk_t)^2 + \frac{R_{\textrm{ext}, T}}{T} + \frac{1}{T} \sum_{t=1}^T \sum_{i=1}^N R^{(i)}_{i,T_i} + \frac{1}{N}.
\end{align*}

Typically, $R_{\textrm{ext}, T} = O(1/\sqrt{T})$, and we therefore get the same $O(1/\sqrt{T})$ regret for each $\pk$ as we did when $K=1$.

The dependence on $K$ depends on the external regret minimization algorithm that we use; it can be made as low as $O(\sqrt{(\log K) / T})$. Note that we factored out the dependence on $K$ from our framework, and so our dependence on $K$ can be made equal to that of the current best algorithm.

